From Dialogue to Diagnostic Hypotheses: Evaluating LLM Agents for Psychiatric Assessment

Although LLMs show promising diagnostic reasoning on supplied clinical evidence, their ability to elicit such evidence through free-form psychiatric interviews remains less understood. We evaluate interview quality and diagnostic hypotheses using simulated patients and human participants. For controlled simulation, we introduce PsyCPG, transforming clinical cases into structured patient profiles. On 30 paired cases, experts rate PsyCPG simulations higher in quality than raw-case role-play (4.50 versus 3.83/5). We introduce PsyCIDRA, a dual-agent framework: its interviewer agent uses a notepad tool, expert-written skills, and ICD-11 reference tools to guide interviews; its diagnostic agent analyzes the transcript and produces a report for expert review, ranking differential diagnoses with supporting, conflicting, and missing evidence. Across four models and 53 development cases, PsyCIDRA achieves higher observed diagnostic agreement than direct prompting. On 81 held-out simulated cases, exact-code rank-1 accuracy reaches 60.5% versus 51.9%. We conduct 101 interviews with human participants; two psychologists, blinded to interview condition and model reports, independently assess interview quality and transcript-supported hypotheses. In separate arms, PsyCIDRA agrees with experts on whether to issue a hypothesis in 79.6% of cases versus 65.4% for direct prompting. This study provides an empirical basis for understanding and evaluating LLM agents in free-form psychiatric interviewing.

==> generated/app_a_diagnosis_pairs.tex <==
\begin{tabular}{lrrrr}
\toprule
Endpoint & Raw case & PsyCPG & Gains & Losses \\
\midrule
Reference code ranked first & 24/30 & 29/30 & 5 & 0 \\
Reference code anywhere in list & 26/30 & 29/30 & 3 & 0 \\
\bottomrule
\end{tabular}


==> generated/app_d_budget.tex <==
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lrrrrrr@{}}
\toprule
Interview / diagnosis & \multicolumn{2}{c}{R1 (/53)} & \multicolumn{2}{c}{Coverage (/53)} & \multicolumn{2}{c}{Tokens (M)} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& 16 & 24 & 16 & 24 & 16 & 24 \\
\midrule
Direct / Direct & 39 & 40 & 42 & 43 & 5.82 & 10.47 \\
Direct / PsyDARA & 40 & 40 & 42 & 41 & 7.10 & 11.93 \\
PsyCIRA / Direct & 44 & 41 & 44 & 42 & 25.22 & 38.69 \\
PsyCIRA / PsyDARA & 44 & 44 & 45 & 46 & 26.48 & 40.10 \\
\bottomrule
\end{tabular*}


==> generated/app_d_quality_domains.tex <==
\begin{tabular}{lrr}
\toprule
Score or domain & Direct & PsyCIRA \\
\midrule
AIIE overall (/5) & 3.73 & 3.98 \\
Diagnostic inquiry & 4.02 & 3.98 \\
Clinical risk & 4.15 & 4.00 \\
Rapport & 3.58 & 3.98 \\
Interview flow & 3.40 & 3.97 \\
CCSS-S overall (/3) & 2.39 & 2.62 \\
Collaboration & 2.60 & 2.71 \\
Structuring/exploration & 2.13 & 2.47 \\
\bottomrule
\end{tabular}


==> generated/app_e_availability.tex <==
\begin{tabular}{@{}lrr@{}}
\toprule
Available data & Direct & PsyCIRA \\
\midrule
Demographics & 52/52 & 49/49 \\
History form & 43/52 & 44/49 \\
Experience form & 43/52 & 44/49 \\
Any experience rating & 42/52 & 42/49 \\
All six ratings & 39/52 & 41/49 \\
\bottomrule
\end{tabular}


==> generated/app_e_codes.tex <==
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{.49\linewidth}rrrrr@{}}
\toprule
Expert primary reference & $n$ & \multicolumn{2}{c}{Direct} & \multicolumn{2}{c}{PsyDARA} \\ \cmidrule(lr){3-4}\cmidrule(l){5-6} & & R1 & Any & R1 & Any \\
\midrule
6B43 Adjustment disorder & 17 & 14 & 16 & 14 & 15 \\
6A70 Single-episode depression & 9 & 5 & 8 & 6 & 9 \\
6B00 Generalized anxiety & 7 & 4 & 7 & 5 & 7 \\
6A71 Recurrent depression & 3 & 0 & 0 & 1 & 1 \\
6A72 Dysthymia & 3 & 1 & 2 & 1 & 2 \\
6A05 ADHD & 1 & 1 & 1 & 1 & 1 \\
6A73 Mixed depressive/anxiety & 1 & 0 & 0 & 0 & 0 \\
6B40 Post-traumatic stress & 1 & 0 & 1 & 0 & 1 \\
6B66 Depersonalization/derealization & 1 & 1 & 1 & 1 & 1 \\
\midrule Total & 43 & 26 & 36 & 29 & 37 \\
\bottomrule
\end{tabular}


==> generated/app_e_comfort_distress.tex <==
\begin{tabular}{lrrr}
\toprule
Agreement & Direct & PsyCIRA & All \\
\midrule
Comfort and distress & 5 & 6 & 11 \\
Comfort only & 25 & 27 & 52 \\
Distress only & 3 & 1 & 4 \\
Neither & 6 & 7 & 13 \\
\midrule
Paired respondents & 39 & 41 & 80 \\
\bottomrule
\end{tabular}


==> generated/app_e_demographics.tex <==
\begin{tabular}{@{}lrr@{}}
\toprule
Characteristic & Direct & PsyCIRA \\
\midrule
\multicolumn{3}{l}{\emph{Gender}} \\
Woman & 27 & 32 \\
Man & 25 & 16 \\
Declined & 0 & 1 \\
\multicolumn{3}{l}{\emph{Age}} \\
18--24 & 13 & 13 \\
25--34 & 18 & 17 \\
35--44 & 5 & 8 \\
45--54 & 10 & 7 \\
55--64 & 5 & 3 \\
65+ & 1 & 1 \\
\multicolumn{3}{l}{\emph{Education}} \\
High school or below & 0 & 4 \\
Bachelor's & 15 & 21 \\
Master's & 30 & 22 \\
Doctorate & 7 & 2 \\
\bottomrule
\end{tabular}


==> generated/app_e_differentials.tex <==
\begin{tabular}{@{}lrrr@{}}
\toprule
Reviewers & $n$ & \multicolumn{2}{c}{AI issued} \\ with candidates & & Direct & PsyDARA \\
\midrule
Neither & 24 & 6 & 4 \\
One & 22 & 14 & 6 \\
Both & 12 & 11 & 9 \\
\midrule Total & 58 & 31 & 19 \\
\bottomrule
\end{tabular}


==> generated/app_e_history.tex <==
\begin{tabular}{@{}lrrrrr@{}}
\toprule
History & Never/no & Past & Current & Other & Missing \\
\midrule
Assessment & 45 & 36 & 2 & 2 & 16 \\
Therapy & 44 & 29 & 8 & 1 & 19 \\
Diagnosis & 65 & 6 & 7 & 5 & 18 \\
Medication & 58 & 11 & 12 & 1 & 19 \\
\bottomrule
\end{tabular}


==> generated/app_e_paired.tex <==
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Endpoint & $n$ & Both & Direct only & PsyDARA only & Neither \\
\midrule
Decision agreement & 101 & 69 & 1 & 12 & 19 \\
Reference rank 1 & 43 & 24 & 2 & 5 & 12 \\
Reference coverage & 43 & 35 & 1 & 2 & 5 \\
\bottomrule
\end{tabular}


==> generated/app_e_reviewer_descriptive.tex <==
\begin{tabular}{lrrrrrr}
\toprule
 & \multicolumn{3}{c}{Reviewer 1} & \multicolumn{3}{c}{Reviewer 2} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Score & Direct & PsyCIRA & $\Delta$ & Direct & PsyCIRA & $\Delta$ \\
\midrule
AIIE overall & 3.76 & 3.99 & $+0.23$ & 3.74 & 3.67 & $-0.07$ \\
Diagnostic inquiry & 3.77 & 3.87 & $+0.09$ & 3.60 & 3.19 & $-0.41$ \\
\quad Medical/biological rule-outs & 3.79 & 3.82 & $+0.03$ & 3.35 & 2.27 & $-1.08$ \\
Risk recognition & 3.92 & 3.98 & $+0.06$ & 4.02 & 3.69 & $-0.33$ \\
Rapport & 3.77 & 4.08 & $+0.31$ & 3.86 & 3.97 & $+0.11$ \\
Interview flow & 3.68 & 4.05 & $+0.37$ & 3.72 & 3.96 & $+0.24$ \\
\midrule
CCSS-S overall & 2.58 & 2.77 & $+0.19$ & 2.44 & 2.52 & $+0.08$ \\
\bottomrule
\end{tabular}


==> generated/app_e_safety_by_arm.tex <==
\begin{tabular}{@{}lrr@{}}
\toprule
Concern & Direct & PsyCIRA \\
 & Either/both & Either/both \\
\midrule
Treatment recommendation & 1 / 0 & 0 / 0 \\
Crisis neglect & 0 / 0 & 2 / 1 \\
Irrelevant data request & 1 / 0 & 1 / 0 \\
\midrule
Any concern & 2 / 0 & 3 / 1 \\
\bottomrule
\end{tabular}


==> generated/app_e_selfreport_decisions.tex <==
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{.43\linewidth}rrrr@{}}
\toprule
Professional diagnosis & $n$ & Experts & Direct & PsyDARA \\
\midrule
Current diagnosis or follow-up & 7 & 5 & 7 & 6 \\
Past diagnosis; no active follow-up & 6 & 4 & 6 & 6 \\
Under evaluation; no diagnosis & 1 & 1 & 1 & 1 \\
No professional diagnosis & 65 & 21 & 45 & 34 \\
Unsure or declined & 4 & 3 & 4 & 4 \\
Unanswered & 18 & 9 & 11 & 10 \\
\midrule
All participants & 101 & 43 & 74 & 61 \\
\bottomrule
\end{tabular}


==> generated/app_e_tokens.tex <==
\begin{tabular}{@{}lrrrrr@{}}
\toprule
Stage/mode & $n$ & Input & Cached input & Output & Total \\
\midrule
Direct interview & 52 & 17.6k & 11.1k & 2.4k & 20.0k \\
PsyCIRA interview & 49 & 258.6k & 242.7k & 2.7k & 261.4k \\
Direct report & 101 & 2.4k & 0.0k & 0.3k & 2.7k \\
PsyDARA report & 101 & 21.0k & 7.3k & 2.0k & 22.9k \\
\bottomrule
\end{tabular}

